TELeR: A General Taxonomy of LLM Prompts for Benchmarking Complex Tasks

While LLMs have shown great success in understanding and generating text in traditional conversational settings, their potential for performing ill-defined complex tasks is largely under-studied. Indeed, we are yet to conduct comprehensive benchmarking studies with multiple LLMs that are exclusively focused on a complex task. However, conducting such benchmarking studies is challenging because of the large variations in LLMs' performance when different prompt types/styles are used and different degrees of detail are provided in the prompts. To address this issue, the paper proposes a general taxonomy that can be used to design prompts with specific properties in order to perform a wide range of complex tasks. This taxonomy will allow future benchmarking studies to report the specific categories of prompts used as part of the study, enabling meaningful comparisons across different studies. Also, by establishing a common standard through this taxonomy, researchers will be able to draw more accurate conclusions about LLMs' performance on a specific complex task.

==> Sandbox/Tables/intersection_examples.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Reward/Kendall Table

\begin{table*}[!htb]\small
% \begin{subtable}[h]{\textwidth}
\centering


\ra{1.2}
\adjustbox{max width=\textwidth}{%
\begin{tabular}{C{3.5cm} | C{3.5cm} | C{3.5cm} | C{5.5cm}} %| m{0.8cm} | m{2cm}}
\toprule
\multicolumn{4}{c|}{\textbf{Narrative Pair Example \# 1}}\\
\hline
\multicolumn{2}{c|}{\textbf{Narrative 1:} $\mathbf{N_1}$} &
\multicolumn{2}{c}{\textbf{Narrative 2:} $\mathbf{N_2}$} \\
\hline
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Sample 1
\multicolumn{2}{C{8cm}|}{
% %% -----------------------------------------
%% D1
\hlgreen{
WASHINGTON -- U.S. intelligence and law enforcement agencies have confirmed that President Donald Trump's campaign aides and associates had constant contact with Russian intelligence officials before the election, directly contradicting public statements made by top administration officials. 
}
On Jan. 15, shortly before Trump took office, Vice President Mike Pence repeatedly said on television that there were zero contacts between the campaign and Russian officials. 
$\mathbf{\dotso}$

\hlgreen{
Pence also answered "of course not" when asked a similar question that day by "Fox News Sunday" host Chris Wallace
$\mathbf{\dotso}$

Trump himself also denied these interactions
$\mathbf{\dotso}$

}
"There's nothing that would conclude me that anything different has changed with respect to that time period," Spicer said. 
$\mathbf{\dotso}$

%% -----------------------------------------
} &
\multicolumn{2}{C{8cm}}{
%% -----------------------------------------
%% D2
\hlgreen{
President Trump said Wednesday that new reports saying his associates had contact with Russian officials during last year's campaign are "non-sense"} and accused the U.S. intelligence community of illegally leaking information to news outlets. 
\hlgreen{
"This Russian connection non-sense} is merely an attempt to cover-up the many mistakes made in Hillary Clinton's losing campaign," Mr. Trump tweeted. 
$\mathbf{\dotso}$

Among those supposedly communicating with Russian nationals was former Trump campaign chairman Paul Manafort, the report said. 
\hlgreen{Mr. Manafort denied that he ever knowingly talked to any intelligence official "or anyone}
%% -----------------------------------------
} \\
\hline
\multicolumn{4}{c}{\textbf{Reference Overlap Summaries}} \\\hline
  \multicolumn{1}{c}{\textbf{A\textsubscript{1}}} &
  \multicolumn{1}{c}{\textbf{A\textsubscript{2}}} &
  \multicolumn{1}{c}{\textbf{A\textsubscript{3}}} &
  \multicolumn{1}{c}{\textbf{AllSides}}
  \\


\hline
%% A1
President Trump and the Trump administration deny allegations that advisers close to Trump were in constant communication during the campaign with Russians known to US intelligence.
&
%% A2
Trump denied climas that advisers close to him were in "constant communication during the campaign with Russians known to US intelligence.
&
%% A3
Donald Trump and his group claimed that there is no contact with Russian officials during his last year's campaign. 
&
%% A4
Russian intelligence officials made repeated contact with members of President Trump's campaign staff, according to new reports that cite anonymous U.S. officials. American agencies were concerned about the contacts but haven't seen proof of collusion between the campaign and the Russian security apparatus.
\\
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\midrule
\midrule


\multicolumn{4}{c|}{\textbf{Narrative Pair Example \# 2}}\\\hline
\multicolumn{2}{c|}{\textbf{Narrative 1:} $\mathbf{N_1}$} &
\multicolumn{2}{c}{\textbf{Narrative 2:} $\mathbf{N_2}$} \\
\hline

\multicolumn{2}{C{8cm}|}{
% %% -----------------------------------------
%% D1
John McCain is out of McConnell's clutches for a week or two. 
\hlgreen{
While Sen. John McCain remains in Arizona recovering from Friday's craniotomy, surgery to remove a 5 cm blood clot from above his left eye}, business will not go on as usual in Washington. 
\hlgreen{
Majority Leader Mitch McConnell, who has to have every Republican senator voting to have a prayer of passing Trumpcare, has postponed the vote for the week or two (more likely two) that McCain's recovery will take.
}
That means there's more time for opponents to fight this thing, from the side of all of us trying to keep 22 million people from losing insurance and from the other side. 
$\mathbf{\dotso}$

\hlgreen{With both Paul and Sen. Susan Collins (R-ME) solid "no" votes on the bill}, opponents only need one more out of the eight or so who've expressed reservations about the bill and the secretive, exclusive process McConnell
%% -----------------------------------------
} &
\multicolumn{2}{C{8cm}}{
%% -----------------------------------------
%% D2
\hlgreen{WASHINGTON - The Republican effort to repeal and replace Obamacare faces a major setback as Sen. John McCain, R-Ariz., left the nation's capital for surgery on his eye. 
Over the weekend, Senate Majority Leader Mitch McConnell, R-Ky., announced the scheduled Better Care Act vote would be delayed indefinitely because of McCain's absence.}
Subsequently, the Congressional Budget Office (CBO) also delayed its analysis of the bill. 
\hlgreen{With two Republican senators opposed to the measure, McConnell needs as least 50 "yes" votes to pass it.}
\hlgreen{Sen. Rand Paul, R-Ky., says the bill, which keeps taxes on investments and other pieces of Obamacare, doesn't go far enough. 
Moderate Sen. Susan Collins, R-Maine, is also withholding her support because it would slow the rate of growth in spending on Medicaid.}
$\mathbf{\dotso}$

%% -----------------------------------------
} \\
\hline
\multicolumn{4}{c}{\textbf{Reference Overlap Summaries}} \\\hline
\multicolumn{1}{c}{\textbf{A\textsubscript{1}}} &
  \multicolumn{1}{c}{\textbf{A\textsubscript{2}}} &
  \multicolumn{1}{c}{\textbf{A\textsubscript{3}}} &
  \multicolumn{1}{c}{\textbf{AllSides}}
  \\


\hline

%% A1
Sen. John McCain remains in Arizona recovering from eye surgery. Senate Majority Leader Mitch  McConnell postponed the vote due to McCain's absence. Two Republican senators opposed to the bill. Possibility of bill failing.
&
%% A2
Sen. John McCain remains unavailable because of the surgery on his eye. Senate Majority Leader Mitch McConnell delayed the vote in his absence. Sen. Rand Paul and Sen. Susan Collins said "no" votes on the bill.
&
%% A3
Senate Majority Leader Mitch McConnell, R-Ky., announced the scheduled health care vote would be delayed indefinitely because of McCain's absence.
&
%% A4
Senate Majority Leader Mitch McConnell, R-Ky., announced the scheduled Better Care Act vote would be delayed indefinitely because of McCain's absence.
\\
\bottomrule
\end{tabular}
}
\caption{Some examples of \textit{SOS} references from 3 human annotators (\textbf{A\textsubscript{i}}) and the AllSides ``theme-description'' for a given narrative pair $\{N_1, N_2\}$. 
($\mathbf{\dotso}$) denotes some sentences which for not shown for brevity. More examples can be found over \href{https://karmake2.github.io/publications/}{here}. Having multiple human annotators is critical to perform robust evaluation, but it is laborious and time-consuming on humans' part. This also shows that the lack of available datasets is a huge challenge for the SOS task. 
% ($\mathbf{\dotso}$) denotes some the sentences which for not shown for brevity.
}
\label{table:qualitative_analysis}
\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> Sandbox/Tables/prompt_example.tex <==
\begin{table}[]
% \caption{ChatGPT and Bard has different understanding of conflicts in the two narratives}
% \label{table:prompt_example}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|cl|}
\hline
\multicolumn{1}{|c|}{Narrative 1} &
  \multicolumn{1}{c|}{Narrative 2} \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}.....The indictment against Paul Manafort and his former \\ business associate Rick Gates has been unsealed and \\ leading the list of charges is "Conspiracy Against the\\  United States" and money laundering. "In order to\\  hide Ukraine payments from United States authorities,"\\  the indictment reads.....\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}...Although the indictment with the details has not been unsealed, \\ according to reports Manafort is facing charges on tax fraud and \\ other white collar crimes completely unrelated to the 2016 \\ presidential election. His former business partner, Rick Gates, is \\ also expected to surrender to authorities. Both were told to turn \\ themselves in or face arrest.....\end{tabular} \\ \hline
\multicolumn{2}{|c|}{Prompt: Read the first narrative, then read the second narrative, and highlight the information that two narratives are in conflict with each other} \\ \hline
\multicolumn{1}{|c|}{\textbf{ChatGPT Output}} &
  \multicolumn{1}{c|}{Bard Output} \\ \hline
\multicolumn{1}{|l|}{\begin{tabular}[c]{@{}l@{}}After reviewing both narratives, it appears that \\ there is no conflict or contradiction between the two. \\ Instead, the second narrative provides additional information \\ and updates on the situation mentioned in the first narrative, \\ specifically on the charges against Paul Manafort and his \\ surrender to the authorities. Both narratives mention the charges \\ of money laundering and conspiracy against the United States, \\ but the second narrative adds that the charges also include tax fraud \\ and other white-collar crimes unrelated to the 2016 presidential \\ election. Therefore, the second narrative complements and \\ expands on the information presented in the first narrative \\ without contradicting it.\end{tabular}} &
  \begin{tabular}[c]{@{}l@{}}The two narratives conflict in the following ways:\\  --The first narrative states that Manafort and Gates were charged with \\      "Conspiracy Against the United States" and money laundering. \\  --The second narrative states that Manafort is facing charges on tax fraud\\      and other white collar crimes completely unrelated to the 2016 presidential election.\\  --The first narrative states that the indictment was unsealed, while the second \\      narrative states that the indictment has not been unsealed.\\  --The first narrative states that Manafort and Gates laundered money through\\    scores of United States and foreign corporations, partnerships, and bank accounts. \\  --The second narrative does not mention any specific allegations of money laundering.\\ It is possible that the two narratives are simply reporting different aspects of\\  the same case. ...\end{tabular} \\ \hline
\end{tabular}%
}
\caption{ChatGPT and Bard has different understanding of conflicts in the two narratives}
\label{table:prompt_example}
\end{table}

==> Sections/2General.tex <==
\section{Datas-set}\label{sec:Motivation}
As we have discussed before, the SOS task is a newly introduced NLP mission, and its benchmark data-set has recently been made available. In this section, we will briefly outline the statistical information regarding the benchmark data-set. More details can be seen here ~\cite{bansal2022semantic}.

Table \ref{table:allSide} gives an overview of the dataset statistics
created by crawling from AllSides.com, which consists of news articles covering 2, 925 events in total and also has a minimum length of “theme description” to be 15 words.



\begin{table*}
    \begin{tabular}{|lllll|}
    \hline
    \multicolumn{5}{|c|}{AllSides Dataset: Statistics} \\ \hline
    \multicolumn{1}{|l|}{Split} & \multicolumn{1}{l|}{\#words(per docs)} & \multicolumn{1}{l|}{\#sents(per docs)} & \multicolumn{1}{l|}{\#word (per reference)} & \#sents (per reference) \\ \hline
    \multicolumn{1}{|l|}{Train} & \multicolumn{1}{l|}{1613.69} & \multicolumn{1}{l|}{66.70} & \multicolumn{1}{l|}{67.30} & 2.82 \\ \hline
    
    \multicolumn{1}{|l|}{Test} & \multicolumn{1}{l|}{959.80} & \multicolumn{1}{l|}{44.73} & \multicolumn{1}{l|}{65.46/38.06/21.72/32.82} & 3.65/2.15/1.39/1.52 \\ \hline
    \end{tabular}
    \caption{Statistics for the Training and Testing dataset. Two input narratives are concatenated to compute the statistics. Four numbers for reference (\#words/\#sents) in the Test split correspond to the 4 reference overlap summaries. Our test dataset contains 137 samples, wherein each sample has 4 ground truth references. Out of these 4 references, one summary is provided by AllSides, and 3 of them were manually written by 3 human annotators. Thus generated 3*137 = 411 references in total.}
    \label{table:allSide}
\end{table*}



==> Sections/3ExperimentalDesign.tex <==
\section{Experiment Design and Results}\label{sec:Experiment}

\subsection{Prompt Design}
Our prompt design taxonomy is based on multiple previous research~\cite{wei2022chain, zhou2022least}. As a human, finding the semantic overlap summary of two alternative narratives can be break down into a series of simple steps:


\begin{enumerate}[leftmargin=*,itemsep=0ex,partopsep=0ex,parsep=0ex]

\item Read the first narrative.

\item Read the second narrative.

\item Find the common information that appears in both two narratives.

\item Summarize the information found in the last step.

\end{enumerate}


However, the above-mentioned step encompasses crucial aspects such as defining intersection/complementary information where these set-like intersection operators were envisioned by ~\cite{karmaker2018sofsat}. We use prompts to locate questions related to "conflict" in addition to retrieving common information. It's important to note that this is different from using an intersection/common operator because two narratives may provide distinct and conflicting perspectives on a shared issue. The purpose of this prompt is to evaluate the capability of LLMs to comprehend and define political conflicts.

In short, we design the prompts from "least to most" strategy where the \textit{least} is just a simple request and the\textit{ most} describes each step to solve the corresponding task. Table~\ref{table:prompts_table} concludes the prompts we use in this experiment. We have four tasks in total: 1) holistic summary of two narratives; 2) overlapping of two narratives; 3) unique of each narrative; and 4) conflicts between two narratives. For each task, we have one brief and one detailed prompt for LLMs. The detailed prompt can be considered as an explanation of the brief prompt. For instance, to solve the "unique" task, the brief prompt can be "\textit{Highlight the unique information of each narrative}" while the detailed prompt would provide an instruction to LLM , e.g., "\textit{Read the first narrative, then read the second narrative, highlight the unique
information that only in each narrative}". 



% Each prompt is mainly divided into two types, the first two are only looking for common and conflict, and the third design is to put the first two commands in the same one. Meanwhile, we use a difficult level to indicate the complexity of each prompt where 0 means the simplest complexity and 2 is the most complicated one. Specifically, we use the same prompt to stimulate two LLMs and compare the responses from the perspective of human understanding.

% \caption{Prompt for ChatGPT and Bard. Level indicates the complexity of the prompt}
% \label{fig:prompts_table}



\begin{table*}
% \caption{Prompt for ChatGPT and Bard. We designed "brief" and "Details" prompts for same purpose}
% \label{table:prompts_table}
\resizebox{\textwidth}{!}{%
\begin{tabular}{|l|l|l|}
\hline
\multirow{2}{*}{Holistic}    & Brief   & Create a summary                                                       \\ \cline{2-3} 
                             & Details & Create a summary highlights the  information  of two given  narratives \\ \hline
\multirow{2}{*}{Overlapping} & Brief   & Highlight  the overlapping between given two narratives                \\ \cline{2-3} 
 &
  Details &
  \begin{tabular}[c]{@{}l@{}}Read the first narrative, then read the second narrative, summarize the\\ content appear in both\end{tabular} \\ \hline
\multirow{2}{*}{Unique}      & Brief   & Highlight the unique information of each narrative                     \\ \cline{2-3} 
 &
  Details &
  \begin{tabular}[c]{@{}l@{}}Read the first narrative, then read the second narrative, highlight the unique \\ information that only in each narrative\end{tabular} \\ \hline
\multirow{2}{*}{Conflicts}   & Brief   & Highlight the conflicts of two narratives                              \\ \cline{2-3} 
 &
  Details &
  \begin{tabular}[c]{@{}l@{}}Read the first narrative, then read the second narrative, highlight the information that two \\ narratives are in conflict with each other\end{tabular} \\ \hline
\end{tabular}%
}
\caption{Prompt for ChatGPT and Bard. We designed "brief" and "Details" prompts for same purpose}
\label{table:prompts_table}
\end{table*}







\subsection{Experimental Results}
Both ChatGPT and Bard can generate reasonable responses for prompts that are looking for "common" information with different detail levels.  For instance, while using "create a summary" as the prompt, ChatGPT generated the response that first describes the common information of two narratives, then  depict two narratives individually. However, Bard will respond in a more comprehensive way: while it also gives an overall summarization of two narratives and two individual descriptions of each one. It also compares the two narratives from diverse perspectives. Here is a sentence of Bard result: \textit{Both narratives are important because they provide information about the charges against Manafort} which we can see Bard is trying to analyze the narratives. 

The second and more interesting observation is related to prompts that are looking for "conflict". When using the three "conflict" prompt with a detailed version, we can see ChatGPT only trying to find the conflict between two narratives. In some cases, ChatGPT would respond as \textit{"There are no conflicts between the two narratives."}. Whereas the answer of Bard is still more comprehensive, although prompts are essentially designed to only find the conflicts between two narratives,  Bard not only concludes the conflict between two narratives, it also retrieves the conflict within each narrative.
While using the \textit{"Step by step"} prompt, Bard even explains how it follows each step and the temporary understanding of each step, then it explained that finally use the previous result to combine the final disagreement. When solving the holistic task, ChatGPT essentially combines each individual result together. However, Bard can generate a different understanding compared to its individual prompt result.
The other two minor observations are: 1) the response of ChatGPT is always shorter than the one of Bard; 2) Bard would make the response more structured, e.g. using bullet points, see Table~\ref{table:prompt_example}.
